Inertial Block Proximal Methods for Non-Convex Non-Smooth Optimization

We propose inertial versions of block coordinate descent methods for solving non-convex non-smooth composite optimization problems. Our methods possess three main advantages compared to current state-of-the-art accelerated first-order methods: (1) they allow using two different extrapolation points to evaluate the gradients and to add the inertial force (we will empirically show that it is more efficient than using a single extrapolation point), (2) they allow to randomly picking the block of variables to update, and (3) they do not require a restarting step. We prove the subsequential convergence of the generated sequence under mild assumptions, prove the global convergence under some additional assumptions, and provide convergence rates. We deploy the proposed methods to solve non-negative matrix factorization (NMF) and show that they compete favorably with the state-of-the-art NMF algorithms. Additional experiments on non-negative approximate canonical polyadic decomposition, also known as non-negative tensor factorization, are also provided.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
%\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Inertial Block Mirror Descent Method}{L. T. K. Hien, N. Gillis and P. Patrinos}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Inertial Block Mirror Descent Method for \\ 
Non-Convex Non-Smooth Optimization\thanks{This work was supported by the Fonds de la Recherche Scientifique - FNRS and the Fonds Wetenschappelijk Onderzoek - Vlanderen (FWO) under EOS Project no O005318F-RG47. NG acknowledges the support of the European Research Council (ERC starting grant no 679515). PP was supported by FWO projects: G086318N; G086518N, Research Council KUL: C14/18/068.}
}

% Authors: full names plus addresses.
\author{Le Thi Khanh Hien\thanks{Department of Mathematics and Operational Research, University of Mons, Belgium
  (\email{thikhanhhien.le@umons.ac.be}, \email{nicolas.gillis@umons.ac.be}).}
\and Nicolas Gillis\footnotemark[2] 
\and Panagiotis Patrinos\thanks {Department of Electrical Engineering (ESAT-STADIUS), KU Leuven, Belgium (\email{panos.patrinos@esat.kuleuven.be})}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

